On the Intrinsic Self-Correction Capability of LLMs: Uncertainty and Latent Concept

Large Language Models (LLMs) are able to improve their responses when instructed to do so, a capability known as self-correction. When instructions provide only the task's goal without specific details about potential issues in the response, LLMs must rely on their internal knowledge to improve response quality, a process referred to as intrinsic self-correction. The empirical success of intrinsic self-correction is evident in various applications, but how and why it is effective remains unknown. In this paper, we unveil that intrinsic self-correction can be progressively improved, allowing it to approach a converged state. Our findings are verified in: (1) the scenario of multi-round question answering, by comprehensively demonstrating that intrinsic self-correction can progressively introduce performance gains through iterative interactions, ultimately converging to stable performance; and (2) the context of intrinsic self-correction for enhanced morality, in which we provide empirical evidence that iteratively applying instructions reduces model uncertainty towards convergence, which then leads to convergence of both the calibration error and self-correction performance, ultimately resulting in a stable state of intrinsic self-correction. Furthermore, we introduce a mathematical formulation and a simulation task indicating that the latent concepts activated by self-correction instructions drive the reduction of model uncertainty. Based on our experimental results and analysis of the convergence of intrinsic self-correction, we reveal its underlying mechanism: consistent injected instructions reduce model uncertainty which yields converged, improved performance.

==> sections/applications.tex <==
\section{Practical Applications Inspired by Analytical Insights}
Self-correction is a test-time technique that utilizes instructions to explicitly guide LLMs towards desired behaviors. 
In Section~\ref{sec:main-analysis}, our analytical insights indicate that decreasing model uncertainty and activating positive concepts are two crucial factors jointly contributing to success. 
We hypothesize that the importance of these two factors can be generalized to other applications of LLMs.

To demonstrate the generalizability of these insights, we investigate whether fine-tuning, in addition to self-correction, can also benefit from our findings related to model uncertainty and activated positive concept. 
To this end, we propose a data selection method for task-agnostic gender bias mitigation, implemented through counterfactual data augmentation~\cite{zmigrod-etal-2019-counterfactual}, which involves the following key steps: (1) \textit{activated positive concept}: filtering out sentences without any gendered words and flipping gendered words in the debiasing corpus, (2) \textit{model uncertainty}: calculating the uncertainty of a GPT2-XL\footnote{https://huggingface.co/openai-community/gpt2-xl} model~\cite{kuhn2022semantic} for each sample in the debiasing corpus, and (3) categorizing the debiasing samples into two groups based on their uncertainty and fine-tuning a GPT2-XL model with each group.
To estimate the uncertainty of LLMs regarding a debiasing sample~\cite{kuhn2022semantic}, we incorporate each sample into a question-answer task. 
Following the methodology of~\cite{schick2021self}, we instruct the LLMs to determine whether the sample statement is biased or not.
Further details regarding the experimental setting are provided in Appendix~\ref{app:debiasing}. 
Notably, this data selection method can be easily adapted for various fine-tuning or instructing purposes for LLMs. 
We utilize task-agnostic debiasing as a concrete example to illustrate the effectiveness of this approach.
\begin{figure}[htp]
    \centering
    \includegraphics[width=0.8\textwidth]{figs/section4.pdf}
    \caption{Social bias mitigation for gender stereotypes in GPT2-XL. The language model modeling score (the likelihood of a natural language sequence generated by the given LLMs, the higher the better) and the StereoSet score are reported (the score is shown by the difference to the absolute fair of 0.5, \textbf{the lower the better}). The performance of fine-tuning progress associated with dataset of certainty is shown in blue, and the performance of uncertainty dataset is colored in orange.}
    \label{fig:sec4}
\end{figure}

Figure~\ref{fig:sec4} presents the performance of the language modeling score (the likelihood of a natural language sequence generated by the given LLMs) and the approximated StereoSet score (the difference between the real StereoSet score and the absolute fairness of 0.5), during the fine-tuning process. 
Samples from the certainty group exhibit less uncertainty compared to those from the uncertainty group, although the evaluated LLM are not entirely certain about the certainty group. 
Regarding the language modeling score, the curve for the certainty group consistently remains above that of the uncertainty group across all fine-tuning epochs, indicating that the LLMs are more adept at fitting data they are more certain about. 
Overall, the StereoSet score for the certainty group is lower than that for the uncertainty group, with the gap widening as epochs progress, further proving that higher uncertainty prevent LLMs from an optimal fitting.

Previous studies have shown that the nature of this uncertainty-driven data selection approach is the selected samples are more informative~\cite{coleman2019selection,chatfield1995model}.
With the empirical evidence, we argue that this should be a principle for LLMs as well, and we believe this can used for understanding why self-instruct~\cite{wang2022self} and self-alignment~\cite{sun2024principle} can outperform human-annotated datasets.
The generated samples from LLMs themselves for self-instruct and self-alignment purpose are from the approximated distribution of LLMs' knowledge of pre-training corpora.
Therefore, those samples enjoy lower uncertainty than those annotated by humans.
We leave this for future research.


==> sections/related_work.tex <==
\section{Related work}

\textbf{Uncertainty estimation} is a crucial approach for examining the inner state of machine learning models with respect to an individual sample or a dataset. 
However, estimating uncertainty of LLMs, in the context of language generation, presents unique challenges due to the exponentially large output space and linguistic variants. 
To address these challenges, various estimation techniques are proposed, utilizing token-level entropy~\cite{huang2023look}, sentence-level semantic equivalence~\cite{kuhn2022semantic}, and the distance in the hidden state space~\cite{ren2022out}. 
A reliable uncertainty estimation, which provides the belief of LLMs, is identified as a key step towards safe and explainable NLP systems. 
Notably, our paper does not aim to develop a more faithful and calibrated LLM with unbiased beliefs. 
Instead, we leverage LLMs' uncertainty to interpret self-correction. 



\textbf{Self-correction} is the capability of LLMs that allows them to modify their outputs based on instructions or external feedback. Such ability enables LLMs to adjust their responses for improved accuracy, relevance, and coherence, helping LLMs more effective in various applications. 
Proper-designed self-correction instruction has revealed empirical success in various application scenarios, e.g., machine translation~\cite{chen2023iterative}, code generation~\cite{madaan2023self}, social bias mitigation~\cite{schick2021self}. 
Self-correction techniques~\cite{pan2023automatically} can be roughly categorized into (1) instruction-based one, utilizing vanilla natural language instruction and intrinsic self-correction capability of the LLM (2) external-feedback based one, relying on an external verifier to provide external feedback. Our paper focuses on the intrinsic capability of LLM and the instruction-based self-correction techniques\mao{ while leaving the external ones as the future work}.


